A functional central limit theorem for interacting particle systems on transitive graphs

A finite range interacting particle system on a transitive graph is considered. Assuming that the dynamics and the initial measure are invariant, the normalized empirical distribution process converges in distribution to a centered diffusion process. As an application, a central limit theorem for certain hitting times, interpreted as failure times of a coherent system in reliability, is derived.

==> clti <==
%--------------------------------------------------------------------
%                   Interacting Particle systems
%--------------------------------------------------------------------

%------------------- Livres de base ---------------------------------

@book{Billingsley,
     author = " Billingsley, P.",
     title  = " Probability and measure",
     edition= "3rd",
     year = " 1995",
     publisher = "Wiley, New York"
     }

@book{Biggs,
     author = "Biggs, N.",
     title = "Algebraic Graph Theory",
     year = "1973",
     publisher = "Cambridge University Press"
     }

@book{EthierKurtz,
     author = "Ethier, S. and Kurtz, T.",
     title  = "Markov processes, characterization and convergence",
     year   = "1986",
     publisher = "Wiley, New York"
     }

@book{Feller1,
     author = "Feller, W.",
     title  = "An introduction to probability theory and its applications",
     volume = "I",
     edition= "3rd",
     year   = "1968",
     publisher = "Wiley, London"
     }

@book{Feller2,
     author = "Feller, W.",
     title  = "An introduction to probability theory and its applications",
     volume = "II",
     edition= "2nd",
     year   = "1971",
     publisher = "Wiley, London"
     }

@book{GodsilRoyle,
     author = "Godsil, C. and Royle, G.F.",
     title = "Algebraic Graph Theory",
     year = "2001",
     publisher = "Springer-Verlag, New York"
     }

@book{Liggett,
     author = "Liggett, T.M.",
     title  = "Interacting particle systems",
     year   = "1985",
     publisher = "Springer-Verlag, New York"
     }

@book{Petrov1,
     author = "Petrov, V.V.",
     title  = "Sums of independent Random Variables",
     publisher = "Springer-Verlag, New York",
     year   = "1975"
     }

@book{Petrov2,
     author = "Petrov, V.V.",
     title  = "Limit theorems of probability theory",
     publisher = "Oxford University Press, Oxford",
     year   = "1995"
     }

@book{HolyandRausand,
     author = "H{\o}lyand, A. and Rausand, M.",
     title  = "System reliability theory: models and statistical methods",
     publisher = "Wiley, New York",
     year   = "1994"
     }

@book{AvenJensen,
     author = "Aven, T. and Jensen, U.",
     title  = "Stochastic models in reliability",
     publisher = "Springer-Verlag, New York",
     year   = "1999"
     }

@book{BarlowProschan,
     author = "Barlow, R.E. and Proschan, F.",
     title  = "Mathematical theory of reliability",
     publisher = "SIAM, Philadelphia",
     year   = "1996"
     }

@book{Haas,
     author = "Haas, P.J.",
     title  = "Stochastic {Petri} nets. Modelling, stability, simulation",
     publisher = "Springer-Verlag, New York",
     year   = "2002"
     }

@book{MalyshevMinlos,
     author = "Malyshev, V.A. and Minlos, R.A.",
     title  = "Gibbs random fields: cluster expansions",
     publisher = "Kluwer, Dordrecht",
     year   = "1991"
     }

@book{Pollard,
     author = "Pollard, D.",
     title  = "Convergence of stochastic processes",
     publisher = "Springer-Verlag, New York",
     year   = "1984"
     }

@book{Rosenblatt,
     author = "Rosenblatt, M.",
     title  = "Stationary processes and random fields",
     publisher = "Birkh{\"a}user, Boston",
     year   = "1985"
     }

@book{Saulis,
     author = "Saulis, L. and Statulevicius, V.A.",
     title  = "Limit theorems for large deviations",
     publisher = "Birkh{\"a}user, Boston",
     year   = "1991"
     }

@book{ShorackWellner,
     author = "Shora{\v{c}}k, G.R. and Wellner, J.A.",
     title  = "Empirical Processes with applications to statistics",
     year   = "1986",
     publisher= "Wiley, New York",
     }

@book{Strook,
     author = "Stroock, D.W.",
     title  = "An introduction to the theory of large deviations",
     publisher = "Springer-Verlag, New York",
     year   = "1984"
     }

@proceedings{Tong,
     editor = "Tong, Y.L.",
     title = "Inequalities in Statistics and Probability",
     series = "{IMS} Lecture Notes",
     volume = "5",
     year   = "1984"
     }

@book{DelMoral04,
     author = "{Del Moral}, P.",
     title  = "Feynman-Kac formulae: genealogical and interacting particle
               systems with applications",
     publisher = "Springer-Verlag, New York",
     year   = "2004"
     }

%-------------- Inegalites et faible dependance ---------------------

@incollection{Bakry,
     author = "Bakry, D.",
     title  = "L'hypercontractivit\'e et son utilisation en
                         th\'eorie des semigroupes",
     booktitle = "Ecole d'{\'et\'e} de probabilit{\'e} de Saint-Flour XXII",
     editor = "Bernard, P.",
     year   = "1994",
     series = "L.N. in Mathematics",
     volume = "1581",
     publisher = "Springer-Verlag, New York",
     pages  = "1--114"
     }

@article{BlackwellFreedman,
     author = "D. Blackwell and D. Freedman",
     title  = "The tail $\sigma$-field of a {Markov} chain
                       and a theorem of {Orey}",
     journal= "Ann. Math. Stat.",
     year   = "1964",
     volume = "35",
     pages  = "1291--1295"
     }

@proceedings{ChellappaJain,
     editor = "Chellappa, R. and Jain, A.",
     title  = "Markov random fields:theory and applications",
     year   = "1993",
     publisher= "Academic Press, Boston",
     }

@article{Cohn,
     author = "Cohn, H.",
     title  = "On the tail $\sigma$-field of the countable {Markov} chains",
     journal= "Revue Roumaine de Math\'ematiques Pures et Appliqu\'ees",
     volume = "21",
     number = "6",
     year   = "1976",
     pages  = "667--675"
     }

@book{DemboZeitouni,
     author = "Dembo, A. and Zeitouni, O.",
     title  = "Large deviations techniques and applications",
     edition= "2nd",
     year   = "1998",
     publisher = "Springer-Verlag, New York"
     }

@book{DevroyeLugosi,
     author = "Devroye, L. and Lugosi, G.",
     title  = "Combinatorial methods in density estimation",
     year   = "2001",
     publisher = "Springer-Verlag, New York"
     }

@proceedings{DehlingMikoschSorensen,
     editor = "Dehling, H. and Mikosch, T. and S{\o}rensen, M.",
     title  = "Empirical process techniques for dependent data",
     year   = "2002",
     publisher= "Birkh{\"a}user, Basel",
     }

@book{DeuschelStrook,
     author = "Deuschel, J.D. and Stroock, D.W.",
     title  = "Large deviations",
     publisher = "Academic Press, New York",
     year   = "1989"
     }

@incollection{DobrushinShlosman1,
    AUTHOR = {Dobrushin, R.L. and Shlosman, S.B.},
     TITLE = {Completely analytical {G}ibbs fields},
 BOOKTITLE = {Statistical physics and dynamical systems (K\"oszeg, 1984)},
    SERIES = {Progr. Phys.},
    VOLUME = {10},
     PAGES = {371--403},
 PUBLISHER = {Birkh\"auser Boston},
   ADDRESS = {Boston, MA},
      YEAR = {1985}
}

@incollection {DobrushinShlosman2,
    AUTHOR = {Dobrushin, R. L. and Shlosman, S. B.},
     TITLE = {Constructive criterion for the uniqueness of {G}ibbs field},
 BOOKTITLE = {Statistical physics and dynamical systems (K\"oszeg, 1984)},
    SERIES = {Progr. Phys.},
    VOLUME = {10},
     PAGES = {347--370},
 PUBLISHER = {Birkh\"auser Boston},
   ADDRESS = {Boston, MA},
      YEAR = {1985}
}

@book{Doukhan,
     author = "Doukhan, P.",
     title  = "Mixing: {P}roperties and examples",
     series = "L.N. in Statistics",
     volume = "85",
     year   = "1994",
     publisher = "Springer-Verlag, Berlin"
     }

@article{DedeckerDoukhan,
     author = "Dedecker, J. and Doukhan, P.",
     title  = "A new covariance inequality and applications",
     journal= "Stoch. Proc. Appl.",
     volume = "106",
     number = "1",
     year   = "2003",
     pages  = "63--80"
     }

@article{DoukhanLang,
     author = "Doukhan, P. and Lang, G.",
     title  = "Rates of convergence in the weak invariance principle
               for the empirical repartition process of weakly
               dependent sequences",
     journal= "Stat. Inf. for Stoch. Proc.",
     volume = "5",
     year   = "2002",
     pages  = "199--228"
     }

@article{DoukhanLouhichi,
     author = "Doukhan, P. and Louhichi, S.",
     title  = "A new weak dependence condition and applications to
               moment inequalities",
     journal= "Stoch. Proc. Appl.",
     volume = "84",
     year   = "1999",
     pages  = "313--342"
     }

@article{DoukhanTeyssiere,
     author = "Doukhan, P. and Teyssi{\`e}re, G. and Winant, P.",
     title  = "Vector valued {ARCH($\infty$)}  models",
     journal= "In preparation",
     year   = "2005",
     volume = "",
     pages  = ""
     }

@book{Georgii,
     author = "Georgii, H.O.",
     title  = "Gibbs measures and phase transitions",
     publisher = "de Gruyter, Berlin",
     year   = "1988"
     }

@article{Higuchi,
     author = "Higuchi, Y.",
     title  = "Coexistence of infinite {$(*)$}-clusters. {II}. {I}sing
              percolation in two dimensions",
     journal= "Probab. Th. Rel. Fields",
     volume = "97",
     number = "1-2",
     pages  = "1--33",
     year   = "1993"
}

@book{KindermannSnell,
     author = "Kindermann, R. and Snell, J.L.",
     title  = "Markov random fields and their applications",
     series = "Contemporary Mathematics",
     volume = "1",
     publisher = "AMS, Providence, RI",
     year   = "1980"
     }

@article{Isaac,
     author = "Isaac, R.",
     title  = "The tail $\sigma$-fields of recurrent
                     {M}arkov  Processes",
     journal= "Aplikace Matematiky",
     year   = "1977",
     volume = "22",
     number = "6",
     pages  = "397--408"
     }

@article{Lezaud,
     author = "L{\'e}zaud, P.",
     title  = "Chernoff-type bounds for finite {M}arkov chains",
     journal= "Ann. Applied Probab.",
     year   = "1998",
     volume = "8",
     number = "3",
     pages  = "849--867"
     }

@book{Rio,
     author = "Rio, E.",
     title  = "Th{\'e}orie asymptotique des processus al{\'e}atoires
                                  faiblement d{\'e}pendants",
     series = "Math{\'e}matiques et applications",
     volume = "31",
     year   = "1999",
     publisher = "Springer-Verlag, Berlin"
     }

@article{IgnatyukMalyshev,
     author = "Ignatyuk, I.A. and Malyshev, V.A.",
     title  = "Cluster expansion for locally interacting {Markov} processes",
     journal= "Mosc. Univ. Math. Bull.",
     volume = "43",
     number = "5",
     pages  = "1--6",
     year   = "1988"
}

@article{Ueltschi,
     author = "Ueltschi, D.",
     title  = "Cluster expansions and correlations functions",
     journal= "Moscow Math. Journal",
     volume = "4",
     pages  = "509--520",
     year   = "2004"
}


%-------------------- TCL Champs aleatoires -------------------------

@article{Donsker51,
     author = "Donsker, M.",
     title  = "An invariance principale for certain probability limit theorems",
     journal= "Soviet Math. Dokl.",
     year   = "1975",
     volume = "16",
     pages  = "1141--1145"
     }

@article{Malyshev75,
     author = "Malyshev, V.A.",
     title  = "The central limit theorem for {Gibbsian} random fields",
     journal= "Soviet Math. Dokl.",
     year   = "1975",
     volume = "16",
     pages  = "1141--1145"
     }

@article{Neaderhouser78,
     author = "Neaderhouser, C.C.",
     title  = "Limit theorems for multiply indexed mixing random variables
               with applications to {Gibbs} random fields",
     journal= "Ann. Probab.",
     year   = "1978",
     volume = "6",
     pages  = "207--215"
     }

@article{Newman80,
    author = "Newman, C.M.",
    title  = "Normal Fluctuations and the FKG Inequalities",
    journal= "Comm. Math. Phys.",
    year   = "1980",
    volume = "74",
    number = "2",
    pages  = "119--128"
    }


@article{Bolthausen82,
     author = "Bolthausen, E.",
     title  = "On the central limit theorem for stationary
                              mixing random fields",
     journal= "Ann. Probab.",
     year   = "1982",
     volume = "10",
     pages  = "1047--1050"
     }

@article{Takahata83,
     author = "Takahata, H.",
     title  = "On the rates in the central limit theorem
                   for weakly dependent random fields",
     journal= "Z. Wahrsch. Verw. Gebiete",
     year   = "1983",
     volume = "64",
     pages  = "445--456"
     }

@article{CometsJanzura,
     author = "Comets, F. and Janzura, M.",
     title  = "A central limit theorem for conditionally centered random
               fields with an application to {Markov} fields",
     journal= "J. Appl. Probab.",
     year   = "1998",
     volume = "35",
     pages  = "608--621"
     }

@article{ChenShao04,
     author = "Chen, L.H.Y. and  Shao, Q.M.",
     title  = "Normal approximation under local dependence",
     journal= "Ann. Probab.",
     year   = "2004",
     volume = "32",
     number = "3A",
     pages  = "1985--2028"
     }

@article{KipnisVaradhan,
     author = "Kipnis, C. and Varadhan, S.R.S.",
     title  = "Central limit theorem for additive functionals of
               reversible {Markov} processes and application
               to simple exclusions",
     journal= "Comm. Math. Phys.",
     year   = "1986",
     volume = "104",
     pages  = "1--19"
     }

@article{SethuramanXu,
     author = "Sethuraman, S. and Xu, L.",
     title  = "A central limit theorem for reversible
               exclusion and zero-range particle systems",
     journal= "Ann. Probab.",
     volume = "24",
     number = "4",
     pages  = "1842--1890",
     year   = "1996"
}


%-------------------- Modeles -------------------------

@article{Liggett97,
     author = "Liggett, T.M.",
     title  = "Stochastic models of interacting systems",
     journal= "Ann. Probab.",
     year   = "1997",
     volume = "25",
     number = "1",
     pages  = "1--29"
     }

@article{Shashkin,
     author = "Shashkin, A.",
     title  = "A weak dependence property of a spin system",
     journal= "Preprint",
     year   = "2005"
     }

@article{DurrettLevin94,
     author = "Durrett, R. and Levin, S.A.",
     title  = "Stochastic spatial models: a user's guide
                   to ecological applications",
     journal= "Phil. Trans. Roy. Soc.",
     series = "B",
     year   = "1994",
     volume = "343",
     pages  = "329--350"
     }


@article{Durrett99,
     author = "Durrett, R.",
     title  = "Stochastic spatial models",
     journal= "SIAM Rev.",
     year   = "1999",
     volume = "41",
     pages  = "677--718"
     }

@article{bgy,
     author = "B{\'e}guin, M. and Gray, L. and Ycart, B.",
     title  = "The Load Transfer Model",
     journal= "Ann. Appl. Probab.",
     year   = "1998",
     volume = "8",
     number = "1",
     pages  = "337--353"
     }

@inproceedings{MargoliusWoyczynski01,
     author = "Margolius, B. and Woyczynski, W.A.",
     title  = "Non linear diffusion approximations for queuing networks",
     booktitle = "Stochastics in finite and infinite dimensions",
     editor = "T. Hida et al.",
     year   = "2001",
     publisher = "Birkh{\"a}user, Boston",
     pages  = "259--284"
     }

@article{Bobbioetal98,
     author = "Bobbio, A. and Puliafito, A. and Telek, M. and Trivedi, K.S.",
     title  = "Recent developments in non-markovian stochastic {Petri} nets",
     journal= "J. Systems Circuits and Computers",
     volume = "8",
     number = "1",
     year   = "1998",
     pages  = "119--158"
     }

@article{Forbesetal96,
     author = "Forbes, F. and Fran{\c{c}}ois, O. and Ycart, B.",
     title  = "Stochastic comparison for resource sharing networks",
     journal= "Markov Proc. Rel. Fields",
     volume = "2",
     number = "4",
     year   = "1996",
     pages  = "581--605"
     }

@article{LiuChiou01,
     author = "Liu, T. and Chiou, S.",
     title  = "Application of {Petri} nets to failure analysis",
     journal= "Reliability Engineering and System Safety",
     volume = "57",
     year   = "1997",
     pages  = "129--142"
     }

@article{Volovoi04,
     author = "Volovoi, V.",
     title  = "Modeling of system reliability using {Petri} nets
               with ageing tokens",
     journal= "Reliability Engineering and System Safety",
     volume = "84",
     year   = "2004",
     pages  = "149--161"
     }

@article{ParoissinYcart04,
     author = "Paroissin, C. and Ycart, B.",
     title  = "Central limit theorem for hitting times of
                functionals of {Markov} jump processes",
     journal= "ESAIM P-S",
     volume = "8",
     year   = "2004",
     pages  = "66--75"
     }


%-------------------- Graphes de Cayley -------------------------

@article{HaggstromPeres99,
     author = "H{\"a}ggstr{\"o}m, O. and Peres, Y.",
     title  = "Monotonicity of uniqueness for percolation on {Cayley}
               graphs: all infinite clusters are born simultaneously",
     journal= "Probab. Th. Rel. Fields",
     year   = "1999",
     volume = "113",
     pages  = "273--285"
     }

@article{Haggstrometal00,
     author = "H{\"a}ggstr{\"o}m, O. and Schonmann, R.H. and Steif, J.E.",
     title  = "The {Ising} model on diluted graphs and strong amenability",
     journal= "Ann. Probab.",
     year   = "2000",
     volume = "28",
     number = "3",
     pages  = "1111--1137"
     }

@article{Haggstrometal02,
     author = "H{\"a}ggstr{\"o}m, 0. and Jonasson, J. and Lyons, R.",
     title  = "Explicit isoperimetric constants and phase transitions
                          in the random-cluster model",
     journal= "Ann. Probab.",
     year   = "2002",
     volume = "30",
     pages  = "443--473"
     }

@book{Woess00,
     author = "Woess, W.",
     title = "Random walks on infinite graphs and groups",
     year = "2000",
     publisher = "Cambridge University Press"
     }

@inproceedings{Peres99,
     author = "Peres, Y.",
     title  = "Probability on trees: an introductory climb",
     booktitle = "Ecole d'{\'et\'e} de probabilit{\'e} de Saint-Flour XXVIII",
     editor = "Bernard, P.",
     year   = "1999",
     series = "L.N. in Math.",
     number = "1717",
     publisher = "Springer-Verlag, New York",
     pages  = "193--280"
     }

